Benchmarks for Physical Reasoning AI

Physical reasoning is a crucial aspect in the development of general AI systems, given that human learning starts with interacting with the physical world before progressing to more complex concepts. Although researchers have studied and assessed the physical reasoning of AI approaches through various specific benchmarks, there is no comprehensive approach to evaluating and measuring progress. Therefore, we aim to offer an overview of existing benchmarks and their solution approaches and propose a unified perspective for measuring the physical reasoning capacity of AI systems. We select benchmarks that are designed to test algorithmic performance in physical reasoning tasks. While each of the selected benchmarks poses a unique challenge, their ensemble provides a comprehensive proving ground for an AI generalist agent with a measurable skill level for various physical reasoning concepts. This gives an advantage to such an ensemble of benchmarks over other holistic benchmarks that aim to simulate the real world by intertwining its complexity and many concepts. We group the presented set of physical reasoning benchmarks into subcategories so that more narrow generalist AI agents can be tested first on these groups.

==> tmlr-rebuttal.tex <==

Comment:
I like the idea to propose “clusters” of the benchmarks in Section 3, but I think the current attempt is not successful. First, “cluster” suggests that the benchmarks are going to be partitioned into groups, but this doesn’t seem to happen. It’s actually unclear what benchmarks belong to what clusters, and it certainly seems like some benchmarks are mentioned in multiple cluster discussions. The four clusters themselves also do not seem mutually exclusive, intuitively.

Response:
Thank you for your comments. We agree that this naming can potentially be confusing because clusters are often mutually exclusive. In this section, our goal was to show readers the main types/categories/groups of physical reasoning benchmarks so that they may get a sense of the field’s broadness and be able to investigate their groups of interest further. For example, somebody studying the physical reasoning abilities of large language models will likely begin by looking at the “Language-related Benchmarks” section. We believe the primary source of the confusion you highlighted is caused by clusters often being mutually exclusive. Therefore, to solve this issue, we have renamed section 5 from “Clusters” to “Groups” and replaced all mentions of the word "cluster" with "group."


Comment:
I found it odd to have a “Other Benchmarks” subsection that mentions two other benchmarks, when the main section includes so many already. Why not just add these two to the main?

Response:
Thank you for your comments. We chose to create an "Other Benchmarks" subsection because we believe the benchmarks included here are valuable for assessing the physical reasoning ability of agents under certain conditions but are testing too many confounding variables to be considered pure physical reasoning benchmarks. For the sake of completeness as a survey paper, we felt it was important to make readers aware of their existence while still emphasizing their limitations. To address this confusion, we have added this explanation to the start of the "Other Benchmarks" section.

